Deep Learning Meets Software Engineering: A Survey on Pre-Trained Models of Source Code

Recent years have seen the successful application of deep learning to software engineering (SE). In particular, the development and use of pre-trained models of source code has enabled state-of-the-art results to be achieved on a wide variety of SE tasks. This paper provides an overview of this rapidly advancing field of research and reflects on future research directions.

==> application_table.tex <==
\begin{table*}[htbp]
    \centering
    \caption{List of down-stream SE tasks for evaluating CodePTMs.}
    \label{table:application}
    \resizebox{\textwidth}{!}{
    \begin{threeparttable}
    \begin{tabular}{llllll}
        \toprule
            \textbf{Type}          & \textbf{Down-stream Tasks}                                                                                  & \textbf{Benchmark / Dataset}                            & \textbf{Metrics}\tnote{$\ast$} & \textbf{CodePTMs}                                                                                   & \textbf{SOTA}    \\
        \midrule
            \multirow{16}{*}{Und.} & Variable-Misuse Localization and Repair                                                               & Vasic et al.~\shortcite{vasic2019neural}                & Acc.                    & CuBERT                                                                                                     & CuBERT           \\ \cline{2-6}
                                   & Wrong Binary Operator                                                                                 & Kanade et al.~\shortcite{cubert}                        & Acc.                    & CuBERT                                                                                                     & CuBERT           \\ \cline{2-6}
                                   & Function-Docstring Mismatch                                                                           & Kanade et al.~\shortcite{cubert}                        & Acc.                    & CuBERT                                                                                                     & CuBERT           \\ \cline{2-6}
                                   & Exception Type                                                                                        & Kanade et al.~\shortcite{cubert}                        & Acc.                    & CuBERT                                                                                                     & CuBERT           \\ \cline{2-6}
                                   & \multirow{2}{*}{Code Search / Text-to-Code Retrieval}                                                 & CodeSearchNet                                           & MRR                     & \begin{tabular}[c]{@{}l@{}}CodeBERT, GraphCodeBERT, SynCoBERT,\\SPT-Code\end{tabular}                      & SynCoBERT        \\ \cline{3-6}
                                   &                                                                                                       & CodeXGLUE                                               & MRR / F1 / Acc.         & DOBF, SynCoBERT                                                                                            & SynCoBERT        \\ \cline{2-6}
                                   & \multirow{2}{*}{Code-to-Code Retrieval}                                                               & CLCDSA~\cite{nafi2019clcdsa}                            & Acc. / MRR / NDCG       & CodeDisen                                                                                                  & CodeDisen        \\ \cline{3-6}
                                   &                                                                                                       & POJ-104~\cite{mou2016convolutional}                     & MAP@R                   & OSCAR, SynCoBERT                                                                                           & SynCoBERT        \\ \cline{2-6}
                                   & \multirow{2}{*}{Defect Detection}                                                                     & CodeXGLUE                                               & Acc.                    & C-BERT, PLBART, CoTexT, CodeT5, SynCoBERT                                                                  & CoTexT           \\ \cline{3-6}
                                   &                                                                                                       & Pradel et al.~\shortcite{pradel2018deepbugs}            & Acc.                    & SCELMo                                                                                                     & SCELMo           \\ \cline{2-6}
                                   & \multirow{2}{*}{Clone Detection}                                                                      & BigCloneBench~\cite{svajlenko2014towards}               & F1                      & \begin{tabular}[c]{@{}l@{}}GraphCodeBERT, DOBF, PLBART, CodeT5,\\SynCoBERT\end{tabular}                    & SynCoBERT        \\ \cline{3-6}
                                   &                                                                                                       & CLCDSA~\cite{nafi2019clcdsa}                            & Precision / Recall / F1 & CodeDisen                                                                                                  & CodeDisen        \\ \cline{2-6}
                                   & Code Classification                                                                                   & POJ-104~\cite{mou2016convolutional}                     & MAP@R                   & OSCAR                                                                                                      & OSCAR            \\ \cline{2-6}
                                   & Cloze Test                                                                                            & De Sousa et al.~\shortcite{javabert}                    & Acc.                    & JavaBERT                                                                                                   & JavaBERT         \\ \hline
            \multirow{21}{*}{Gen.} & \multirow{5}{*}{\begin{tabular}[c]{@{}l@{}}Code Summarization /\\ Code Documentation\end{tabular}}    & CodeXGLUE                                               & BLEU                    & \begin{tabular}[c]{@{}l@{}}CodeBERT, DOBF, PLBART, ProphetNet-Code,\\CoTexT, CodeT5, SPT-Code\end{tabular} & \begin{tabular}[c]{@{}l@{}}CodeT5, ProphetNet-Code /\\ ProphetNet-Code, PLBART\tnote{$\dagger$}~\tnote{$\ddagger$}\end{tabular} \\ \cline{3-6}
                                   &                                                                                                       & Haque et al.~\shortcite{haque2020improved}              & BLEU / ROUGE-L          & T5-learning                                                                                                & T5-learning      \\ \cline{3-6}
                                   &                                                                                                       & Hu et al.~\shortcite{hu2018deep}                        & BLEU                    & TreeBERT                                                                                                   & TreeBERT         \\ \cline{3-6}
                                   &                                                                                                       & Hu et al.~\shortcite{hu2018summarizing}                 & BLEU / METEOR           & SPT-Code                                                                                                   & SPT-Code         \\ \cline{3-6}
                                   &                                                                                                       & Miceli et al.~\shortcite{miceli2017parallel}            & BLEU                    & SPT-Code                                                                                                   & SPT-Code         \\ \cline{2-6}
                                   & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Method Naming /\\ Extreme Code Summarization\end{tabular}} & Allamanis et al.~\shortcite{allamanis2016convolutional} & Precision / Recall / F1 & TreeBERT                                                                                                   & TreeBERT         \\ \cline{3-6}
                                   &                                                                                                       & ETH Py150~\cite{raychev2016probabilistic}               & Precision / Recall / F1 & TreeBERT                                                                                                   & TreeBERT         \\ \cline{2-6}
                                   & \multirow{3}{*}{Code Completion}                                                                      & Svyatkovskiy et al.~\shortcite{gpt-c}                   & ROUGE-L / Edit Sim.     & GPT-C                                                                                                      & GPT-C            \\ \cline{3-6}
                                   &                                                                                                       & Liu et al.~\shortcite{cuglm}                            & Acc.                    & CugLM                                                                                                      & CugLM            \\ \cline{3-6}
                                   &                                                                                                       & Alon et al.~\shortcite{alon2020structural}              & Acc@k                   & SPT-Code                                                                                                   & SPT-Code         \\ \cline{2-6}
                                   & \multirow{3}{*}{Code Translation}                                                                     & CodeXGLUE                                               & BLEU / Acc. / CodeBLEU  & \begin{tabular}[c]{@{}l@{}}GraphCodeBERT, PLBART, CodeT5,\\SynCoBERT, SPT-Code\end{tabular}                & CodeT5, SPT-Code\tnote{$\S$} \\ \cline{3-6}
                                   &                                                                                                       & TransCorder~\cite{roziere2020unsupervised}              & Acc                     & DOBF                                                                                                       & DOBF             \\ \cline{3-6}
                                   &                                                                                                       & CLCDSA~\cite{nafi2019clcdsa}                            & BLEU / ROUGE-L / CIDER  & CodeDisen                                                                                                  & CodeDisen        \\ \cline{2-6}
                                   & Code Repair / Bug Fixing                                                                              & CodeXGLUE                                               & BLEU / Acc. / CodeBLEU  & \begin{tabular}[c]{@{}l@{}}GraphCodeBERT, T5-learning, DeepDebug,\\CoTexT, CodeT5, SPT-Code\end{tabular}   & CodeT5           \\ \cline{2-6}
                                   & Mutant Generation                                                                                     & Tufano et al.~\shortcite{tufano2019learning}            & Acc.                    & T5-learning                                                                                                & T5-learning      \\ \cline{2-6}
                                   & Assert Generation                                                                                     & Watson et al.~\shortcite{watson2020learning}            & Acc@k                   & T5-learning                                                                                                & T5-learning      \\ \cline{2-6}
                                   & Code Generation                                                                                       & CodeXGLUE                                               & BLEU / Acc. / CodeBLEU  & PLBART, CoTexT, CodeT5                                                                                     & \begin{tabular}[c]{@{}l@{}}CodeT5 / PLBART,\\ CodeGPT-adapted\tnote{$\dagger$}~\tnote{$\P$}\end{tabular} \\
        \bottomrule
    \end{tabular}
    \begin{tablenotes}
        \footnotesize
        \item[$\ast$] Acc. denotes accuracy, Acc@k, a.k.a. Precision@k, indicates whether the correct answer is among the top $k$ answers predicted by the model. MRR is mean reciprocal rank and NDCG indicates normalized discounted cumulative gain. MAP@R denotes mean average precision at rank $R$, $R=499$ in this dataset. BLEU, ROUGE-L, METEOR, CIDER and CodeBLEU indicate BLEU~\cite{papineni2002bleu}, ROUGE-L~\cite{lin2002manual}, METEOR~\cite{banerjee2005meteor}, CIDER~\cite{vedantam2015cider} and CodeBLEU~\cite{ren2020codebleu} scores, respectively. Edit Sim. is the edit similarity between the correct answer and the prediction.
        \item[$\dagger$] There are some CodePTMs that exploit the alignment between the code and its docstring during pre-training, e.g. by including both in a single input instance (CodeBERT, GraphCodeBERT, SynCoBERT, CoTexT) or using pre-training tasks that translate between the each other (CodeT5). However, in the same way, code summarization/generation are tasks that use the code and correspongding docstring as input and output, or vice versa. It is therefore reasonable to argue that the above CodePTMs are more advantageous to the others, especially on code summarization/generation tasks. Because it means that they have more task-specific manually labeled training data. As a result, on both tasks, we give two sets of SOTAs, one with and one without these CodePTMs, separated by ``/''.
        \item[$\ddagger$] For the first set, ProphetNet-Code is the SOTA on JS, CodeT5 is the SOTA on Java, Python, PHP, Go and Ruby. For the second set, ProphetNet-Code is the SOTA on Java, JS, PHP and Ruby, PLBART is the SOTA on Python and Go.
        \item[$\S$] For accuracy, CodeT5 is SOTA, and SPT-Code is better on BLEU.
        \item[$\P$] PLBART achieves higher BLEU and CodeBLEU, while CodeGPT-adapted is the SOTA on accuracy. CodeGPT-adapted~\cite{lu2021codexglue}, a simple unimodal baseline model, is a GPT-2 model pre-trained on CodeSearchNet.
    \end{tablenotes}
    \end{threeparttable}
    }
\end{table*}

==> codeptms_table.tex <==
\begin{table*}[htbp]
    \centering
    \caption{List of existing CodePTMs.}
    \label{table:codeptms}
    \resizebox{\textwidth}{!}{
    \begin{threeparttable}
    \begin{tabular}{llllll}
        \toprule
            \textbf{CodePTM}                            & \textbf{Architecture}\tnote{$\ast$} & \textbf{Modality}\tnote{$\dagger$} & \textbf{Pre-Training Task}\tnote{$\ddagger$} & \textbf{Dataset}   & \textbf{Dataset Size}                  \\
        \midrule
            CuBERT~\shortcite{cubert}                   & Transformer Encoder & Code                 & MLM + NSP                            & Python from BigQuery                                     & 7.4M Files                             \\
        \hline
            CodeBERT~\shortcite{codebert}               & Transformer Encoder & Code (+ Doc)\tnote{$\S$} & MLM \& RTD                       & CodeSearchNet                                            & \begin{tabular}[c]{@{}l@{}}2.1M Bimodal Functions\\ 6.4M Unimodal Functions\end{tabular} \\
        \hline
            SCELMo~\shortcite{scelmo}                   & LSTM                & Code                 & BiLM                                 & JavaScript from Open Source Projects                     & 150K Files                             \\
        \hline
            GPT-C~\shortcite{gpt-c}                     & Transformer Decoder & Code                 & Forward LM                           & Python, C\#, JS/TS from GitHub                           & 4.7M Files                             \\
        \hline
            C-BERT~\shortcite{c-bert}                   & Transformer Encoder & Code                 & WWM                                  & Top 100 Starred C GiHub Repos                            & 5.8GB                                  \\
        \hline
            GraphCodeBERT~\shortcite{graphcodebert}     & Transformer Encoder & Code + Doc + DFG     & MLM + EP + NA                        & Bimodal CodeSearchNet                                    & 2.1M Functions                         \\
        \hline
            CugLM~\shortcite{cuglm}                     & Transformer Encoder & Code                 & IMLM + NSP + Forward LM              & Java and TS from GitHub                                  & 617K Files                             \\
        \hline
            JavaBERT~\shortcite{javabert}               & Transformer Encoder & Code                 & MLM                                  & Java GitHub Repos                                        & 3M Files                               \\
        \hline
            DOBF~\shortcite{dobf}                       & Transformer         & Code                 & Seq2Seq IMLM                         & Java and Python from BigQuery                            & 11.5M Files                            \\
        \hline
            T5-learning~\shortcite{t5-learning}         & Transformer         & Code \& Doc          & Seq2Seq MLM                          & Java from CodeSearchNet                                  & 1.5M Methods                           \\
        \hline
            PLBART~\shortcite{plbart}                   & Transformer         & Code \& Posts        & DAE (masking / deletion / infilling) & \begin{tabular}[c]{@{}l@{}}Java and Python from GitHub\\ Posts from StackOverflow\end{tabular} & \begin{tabular}[c]{@{}l@{}}680M Functions\\ 47M Posts\end{tabular} \\
        \hline
            ProphetNet-Code~\shortcite{prophetnet-code} & Transformer         & Code \& Doc          & FNP                                  & Bimodal CodeSearchNet                                    & 2.1M Functions                         \\
        \hline
            DeepDebug~\shortcite{deepdebug}             & Transformer         & Code                 & Seq2Seq MLM                          & Java GitHub Repos                                        & 8M Files                               \\
        \hline
            CoTexT~\shortcite{cotext}                   & Transformer         & Code + Doc           & Seq2Seq MLM                          & \begin{tabular}[c]{@{}l@{}}CodeSearchNet\\ Java, Python from BigQuery\end{tabular} & \begin{tabular}[c]{@{}l@{}}6.4M Functions\\ Unknown\end{tabular} \\
        \hline
            TreeBERT~\shortcite{treebert}               & Transformer         & Code + AST Paths     & TMLM + NOP                           & Java and Python from BigQuery                            & 21.3M Files                            \\
        \hline
            OSCAR~\shortcite{oscar}                     & Transformer Encoder & IR + AEI             & MLM + CCL                            & C/C++ GitHub Repos                                       & 500K functions                         \\
        \hline
            CodeDisen~\shortcite{codedisen}             & LSTM                & Code + AST Seq       & VGVAE + CLR + PD + ACP               & CLCDSA~\shortcite{nafi2019clcdsa}                        & 26K Functions                          \\
        \hline
            CodeT5~\shortcite{codet5}                   & Transformer         & Code + Doc           & Seq2Seq MLM / IT / Seq2seq IMLM / BDG& \begin{tabular}[c]{@{}l@{}}CodeSearchNet\\ C, C\# from BigQuery\end{tabular} & 8.35M Functions                        \\
        \hline
            SynCoBERT~\shortcite{syncobert}             & Transformer Encoder & Code + Doc + AST Seq & MLM + IT + TEP + MCL                 & CodeSearchNet                                            & 6.4M Functions                         \\
        \hline
            SPT-Code~\shortcite{spt-code}                & Transformer         & Code + Names + AST Seq & CAP \& MASS \& MNG                 & CodeSearchNet                                            & 6.4M Functions                         \\
        \bottomrule
    \end{tabular}
    \begin{tablenotes}
        \footnotesize
        \item[$\ast$] The difference between ``Transformer Encoder'' and ``Transformer Decoder'' is that the decoder uses an additional mask matrix to prevent future tokens from being seen during auto-regressive generation. Whereas we consider that the decoder must have this matrix, but do not limit the encoder to use it, which is why we classify CugLM (which uses this matrix for its last task but not for the other tasks) as an encoder as well.
        \item[$\dagger$] ``+'' indicates that modalities are concatenated as one input instance, while ``\&'' denotes that the each modality is a standalone input instance.
        \item[$\ddagger$] ``+'' means that the losses of multiple tasks are summed and optimized jointly, ``\&'' indicates that multiple tasks are performed sequentially, while ``/'' means that each pre-training task is performed alternately.
        \item[$\S$] CodeBERT uses ``Code + Doc'' when performing MLM and ``Code'' only when performing RTD.
    \end{tablenotes}
    \end{threeparttable}
    }
\end{table*}

==> table_sota.tex <==
% %第一轮：先阅读所有的CodePTM论文，将里面有的非PTM的模型最好结果填上去，标记模型年份和名字，如果没有就不标。codeptm同样标记名字和具体结果
% %第二轮：对第一轮年份久远的非PTM模型，查找新的非PTM模型作为SOTA
% %在所有指标中选择一个即可
% \begin{table}[t!]
%     \centering
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{llllll}
%     %\begin{tabular}{llllll}
%         \toprule
%             \textbf{Task} & 
%             \textbf{Dataset} &
%             \textbf{Metrics} &
%             \textbf{B-CPTM}&
%             \textbf{B-NonPTM} &
%             \textbf{ER}\\
%         \midrule
%             WB & 
%             K1 - Kanade et al.~\shortcite{cubert} & 
%             Acc &
%             CuBERT 82.30\% & 
%             GREAT~\shortcite{hellendoorn2020global} 73.80\% 2020 &
%             \\
%         \hline 
%             ET & 
%             K1 - Kanade et al.~\shortcite{cubert} & 
%             Acc & 
%             CuBERT 79.12\% & 
%             Transformer 49.56\% 2017 &
%             \\
%         \hline 
%             \multirow{2}{*}{BD} & 
%             D1 - Devign~\shortcite{zhou2019devign} & 
%             Acc & 
%             CodeT5 65.78\% & 
%             code2vec 62.48\% 2019 &
%             \\
%         \cline{2-6} 
%             & 
%             P1 - Pradel et al.~\shortcite{pradel2018deepbugs} & 
%             Acc & 
%             SCELMo & 
%             &
%             \\ 
%         \hline 
%             \multirow{2}{*}{CD} & 
%             B1 - BigCloneBench~\shortcite{svajlenko2014towards} & 
%             F1 & 
%             SynCoBERT 97.4\% & 
%             FA-AST~\shortcite{wang2020detecting} 95\% 2020 & \\ 
%         \cline{2-6} 
%             & 
%             C1 - CLCDSA~\shortcite{nafi2019clcdsa} & 
%             F1 & 
%             CodeDisen 90\% & 
%             Multi-way Tree-LSTM~\shortcite{shido2019automatic} 81\% 2019 & 
%             \\ 
%         \hline 
%             CC & 
%             P2 - POJ-104~\shortcite{mou2016convolutional} & 
%             Acc & OSCAR 2021 98.08%
%             & ProGraML2020 96.62%
%             & 
%             \\
%         \hline 
%             FD &
%             K1 - Kanade et al.~\shortcite{cubert} & 
%             Acc  & 
%             CuBERT 98.09\% & 
%             Transformer 91.02\% 2017 &
%             \\ 
%         \hline 
%             \multirow{2}{*}{CR} &
%             C1 - CLCDSA~\shortcite{nafi2019clcdsa} & 
%             Acc & 
%             CodeDisen 0.316 & 
%             Pontes et al.~\shortcite{pontes2018predicting} 0.166 2018 &
%             \\ 
%         \cline{2-6} 
%             & 
%             P2 - POJ-104~\shortcite{mou2016convolutional} & 
%             MAP@R &
%             SynCoBERT 88.24 & 
%             MISIM~\shortcite{ye2020misim} 82.45 2020 &
%             \\ 
%         \hline 
%             VM & 
%             V1 - Vasic et al.~\shortcite{vasic2019neural} & 
%             Acc & 
%             CuBERT 95.21 & 
%             BiLSTM (Skip-gram) 80.53 &
%             \\ 
%         \hline 
%             CT & 
%             D2 - De Sousa et al.~\shortcite{javabert} & 
%             Acc & 
%             JavaBERT 94.4 & 
%             &
%             \\
%         \hline 
%             \multirow{2}{*}{CS} &
%             C2 - CodeSearchNet~\shortcite{husain2019codesearchnet} & 
%             MRR & 
%             SynCoBERT 74 & 
%             CasCode~\cite{gotmare2021cascaded} 77.95 2021 &
%             \\ 
%         \cline{2-6}   
%             & 
%             C3 - CoSQA~\shortcite{huang2021cosqa} & 
%             Acc & 
%             SynCoBERT 38.1 & 
%             CasCode~\cite{gotmare2021cascaded} 43.98 2021 &
%             \\
%         \hline 
%             \multirow{3}{*}{CP} &
%             S1 - Svyatkovskiy et al.~\shortcite{gpt-c} & 
%             EditSim. & 
%             GPT-C 82.81 & 
%             &
%             \\ 
%         \cline{2-6} 
%             & 
%             L1 - Liu et al.~\shortcite{cuglm} & 
%             Acc & 
%             CugLM 81.91 & 
%             Transformer-XL~\shortcite{dai2019transformer} 71.73 2019 &
%             \\ 
%         \cline{2-6}       
%             & 
%             A1 - Alon et al.~\shortcite{alon2020structural} & 
%             Acc@k (=5) & 
%             SPT-Code 26.57 & 
%             SLM~\shortcite{alon2020structural} 24.77 2020 &
%             \\ 
%         \hline 
%             \multirow{3}{*}{TL} & 
%             C4 - Chen et al.~\shortcite{chen2018tree} & 
%             Acc & 
%             CodeT5 66.40 & 
%             Transformer 35.45 2017 &
%             \\
%         \cline{2-6} 
%             & 
%             T1 - TransCorder~\shortcite{roziere2020unsupervised} & 
%             Acc  & 
%             DOBF 41.8 & 
%             Transformer 34.7 2017 &
%             \\ 
%         \cline{2-6}      
%             & 
%             C1 - CLCDSA~\shortcite{nafi2019clcdsa} & 
%             BLEU & 
%             CodeDisen 29.75 & 
%             Multi-way Tree-LSTM~\shortcite{shido2019automatic} 25.84 2019 &
%             \\ 
%         \hline 
%             BF & 
%             T2 - Tufano et al.~\shortcite{tufano2019empirical} & 
%             Acc & 
%             CodeT5 18.385 & 
%             S2S+COPYSPAN~\shortcite{panthaplackel2021copy} 12.75 2021 &
%             \\ 
%         \hline 
%             MG & 
%             T3 - Tufano et al.~\shortcite{tufano2019learning} & 
%             Acc & 
%             T5-learning 28 & 
%             Tufano~\shortcite{tufano2019learning} 17 2019 &
%             \\ 
%         \hline 
%             AG & 
%             W1 - Watson et al.~\shortcite{watson2020learning} & 
%             Acc@k & 
%             T5-learning 66 & 
%             Watson et al.~\shortcite{watson2020learning} 65 2020 &
%             \\ 
%         \hline 
%             \multirow{5}{*}{SU} &
%             C2 - CodeSearchNet~\shortcite{husain2019codesearchnet} & 
%             BLEU & 
%             CodeT5 19.77 & 
%             Transformer 15.56 2017 &
%             \\ 
%         \cline{2-6}    
%             & 
%             H1 - Haque et al.~\shortcite{haque2020improved} & 
%             BLEU & 
%             T5-learning 21 & 
%             Haque et al.~\shortcite{haque2020improved} 19 2020 &
%             \\ 
%         \cline{2-6}
%             & 
%             H2 - Hu et al.~\shortcite{hu2018deep} & 
%             BLEU & 
%             TreeBERT 20.49 & 
%             Code+GNN+GRU~\shortcite{leclair2020improved} 19.73 2020 &
%             \\ 
%         \cline{2-6}      
%             & 
%             H3 - Hu et al.~\shortcite{hu2018summarizing} & 
%             BLEU & 
%             SPT-Code 49.1 & 
%             AST-Trans~\shortcite{tang2022ast} 48.29 2022 &
%             \\ 
%         \cline{2-6}    
%             & 
%             M1 - Miceli et al.~\shortcite{miceli2017parallel} & 
%             BLEU & 
%             SPT-Code 36.1 & 
%             AST-Trans~\shortcite{tang2022ast} 34.72 2022 &
%             \\ 
%         \hline  
%             \multirow{2}{*}{MN} &
%             A2 - Allamanis et al.~\shortcite{allamanis2016convolutional} & 
%             F1 & 
%             TreeBERT 60.15 & 
%             Code+GNN+GRU~\shortcite{leclair2020improved} 57.54 2020 &
%             \\ 
%         \cline{2-6}       
%             & 
%             E1 - ETH Py150~\shortcite{raychev2016probabilistic} & 
%             F1 & 
%             TreeBERT 39.04 & 
%             Code+GNN+GRU~\shortcite{leclair2020improved} 34.45  &
%             \\ 
%         \hline 
%             CG &
%             C5 - CONCODE~\shortcite{iyer2018mapping} & 
%             Acc & 
%             CodeT5 22.3 & 
%             Iyer et al.~\shortcite{iyer2019learning} 12.20 2019 &
%             \\
%         \bottomrule
%     \end{tabular}
%     }
%     \caption{A categorization of the 18 SE tasks to which CodePTMs have been applied.}
%     \label{table:sota}
%     \vspace{-2mm}
% \end{table}

%第一轮：先阅读所有的CodePTM论文，将里面有的非PTM的模型最好结果填上去，标记模型年份和名字，如果没有就不标。codeptm同样标记名字和具体结果
%第二轮：对第一轮年份久远的非PTM模型，查找新的非PTM模型作为SOTA
%在所有指标中选择一个即可
\begin{table*}[t!]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{llllll}
    %\begin{tabular}{llllll}
        \toprule
            \textbf{Task} & 
            \textbf{Dataset} &
            \textbf{Metrics} &
            \textbf{Best CodePTM}&
            \textbf{Best NonCodePTM} &
            \textbf{ERR}\\
        \midrule
            WB & 
            K1 - Kanade et al.~\shortcite{cubert} & 
            Acc &
            82.30\% (CuBERT~\shortcite{cubert})& 
            73.80\% (GREAT~\shortcite{hellendoorn2020global}) &
            32.4\%
            \\
        \hline 
            ET & 
            K1 - Kanade et al.~\shortcite{cubert} & 
            Acc & 
            79.12\% (CuBERT~\shortcite{cubert})& 
            49.56\% (Transformer~\shortcite{cubert}) &
            58.6\%
            \\
        \hline 
            BD & 
            D1 - Devign~\shortcite{zhou2019devign} & 
            Acc & 
            65.78\% (CodeT5~\shortcite{codet5})& 
            62.48\% (code2vec~\shortcite{coimbra2021using}) &
            8.8\%
            \\
        \hline 
            \multirow{2}{*}{CD} & 
            B1 - BigCloneBench~\shortcite{svajlenko2014towards} & 
            F1 & 
            97.4\% (SynCoBERT \shortcite{syncobert})& 
            95\% (FA-AST~\shortcite{wang2020detecting}) & 
            48\%
            \\ 
        \cline{2-6} 
            & 
            C1 - CLCDSA~\shortcite{nafi2019clcdsa} & 
            F1 & 
            90\% (CodeDisen~\shortcite{codedisen}) & 
            81\% (Multi-way Tree-LSTM~\shortcite{shido2019automatic} ) & 
            47.3\%
            \\ 
        \hline 
            CC & 
            P2 - POJ-104~\shortcite{mou2016convolutional} & 
            Acc & 
            98.08\% (OSCAR~\shortcite{oscar}) & 
            96.62\% (ProGraML~\shortcite{oscar}) & 
            43.2\%
            \\
        \hline 
            FD &
            K1 - Kanade et al.~\shortcite{cubert} & 
            Acc  & 
            98.09\% (CuBERT~\shortcite{cubert}) & 
            91.02\% (Transformer~\shortcite{cubert}) &
            78.7\%
            \\ 
        \hline 
            \multirow{2}{*}{CR} &
            C1 - CLCDSA~\shortcite{nafi2019clcdsa} & 
            Acc & 
            31.6\% (CodeDisen~\shortcite{codedisen})& 
            16.6\% (Pontes et al.~\shortcite{pontes2018predicting} ) &
            17.9\%
            \\ 
        \cline{2-6} 
            & 
            P2 - POJ-104~\shortcite{mou2016convolutional} & 
            MAP@R &
            88.24\% (SynCoBERT~\shortcite{syncobert})& 
            82.45\% (MISIM~\shortcite{ye2020misim} ) &
            32.9\%
            \\ 
        \hline 
            VM & 
            V1 - Vasic et al.~\shortcite{vasic2019neural} & 
            Acc & 
            95.21\% (CuBERT~\shortcite{cubert}) & 
            80.53\% (BiLSTM~\shortcite{cubert}) &
            75.4\%
            \\ 
        \hline 
            CT & 
            D2 - De Sousa et al.~\shortcite{javabert} & 
            Acc & 
            94.4\% (JavaBERT~\shortcite{javabert})& 
            -&
            
            \\
        \hline 
            \multirow{2}{*}{CS} &
            C2 - CodeSearchNet~\shortcite{husain2019codesearchnet} & 
            MRR & 
            74\% (SynCoBERT~\shortcite{syncobert})& 
            77.95\% (CasCode~\shortcite{gotmare2021cascaded}) &
            -17.9\%
            \\ 
        \cline{2-6}   
            & 
            C3 - CoSQA~\shortcite{huang2021cosqa} & 
            Acc & 
            38.1\% (SynCoBERT~\shortcite{syncobert}) & 
            43.98\% (CasCode~\shortcite{gotmare2021cascaded}) &
            -10.5\%
            \\
        \hline 
            \multirow{3}{*}{CP} &
            S1 - Svyatkovskiy et al.~\shortcite{gpt-c} & 
            EditSim. & 
            82.81\% (GPT-C~\shortcite{gpt-c}) & 
            -&
            
            \\ 
        \cline{2-6} 
            & 
            L1 - Liu et al.~\shortcite{cuglm} & 
            Acc & 
            81.91\% (CugLM~\shortcite{cuglm}) & 
            71.73\% (Transformer-XL~\shortcite{dai2019transformer}) &
            36.0\%
            \\ 
        \cline{2-6}       
            & 
            A1 - Alon et al.~\shortcite{alon2020structural} & 
            Acc@k (=5) & 
            26.57\% (SPT-Code~\shortcite{spt-code})& 
            24.77\% (SLM~\shortcite{alon2020structural}) &
            2.4\%
            \\ 
        \hline 
            \multirow{3}{*}{TL} & 
            C4 - Chen et al.~\shortcite{chen2018tree} & 
            Acc & 
            66.40\% (CodeT5~\shortcite{codet5}) & 
            35.45\% (Transformer~\shortcite{plbart}) &
            47.9\%
            \\
        \cline{2-6} 
            & 
            T1 - TransCorder~\shortcite{roziere2020unsupervised} & 
            Acc  & 
            41.8\% (DOBF~\shortcite{dobf}) & 
            34.7\% (Transformer~\shortcite{dobf}) &
            10.9\%
            \\ 
        \cline{2-6}      
            & 
            C1 - CLCDSA~\shortcite{nafi2019clcdsa} & 
            BLEU & 
            29.75\% (CodeDisen~\shortcite{codedisen}) & 
            25.84\% (Multi-way Tree-LSTM~\shortcite{shido2019automatic}) &
            5.3\%
            \\ 
        \hline 
            BF & 
            T2 - Tufano et al.~\shortcite{tufano2019empirical} & 
            Acc & 
            18.385\% (CodeT5~\shortcite{codet5}) & 
            12.75\% (S2S+COPYSPAN~\shortcite{panthaplackel2021copy}) &
            6.5\%
            \\ 
        \hline 
            MG & 
            T3 - Tufano et al.~\shortcite{tufano2019learning} & 
            Acc & 
            28\% (T5-learning~\shortcite{t5-learning}) & 
            17\% (Tufano~\shortcite{tufano2019learning}) &
            13.3\%
            \\ 
        \hline 
            AG & 
            W1 - Watson et al.~\shortcite{watson2020learning} & 
            Acc@k & 
            66\% (T5-learning~\shortcite{t5-learning}) & 
            65\% (Watson et al.~\shortcite{watson2020learning}) &
            2.9\%
            \\ 
        \hline 
            \multirow{5}{*}{SU} &
            C2 - CodeSearchNet~\shortcite{husain2019codesearchnet} & 
            BLEU & 
            19.77\% (CodeT5~\shortcite{codet5}) & 
            15.56\% (Transformer~\shortcite{}) &
            4.9\%
            \\ 
        \cline{2-6}    
            & 
            H1 - Haque et al.~\shortcite{haque2020improved} & 
            BLEU & 
            21\% (T5-learning~\shortcite{t5-learning})& 
            19\% (Haque et al.~\shortcite{haque2020improved}) &
            2.5\%
            \\ 
        \cline{2-6}
            & 
            H2 - Hu et al.~\shortcite{hu2018deep} & 
            BLEU & 
            20.49\% (TreeBERT~\shortcite{treebert})& 
            19.73\% (Code+GNN+GRU~\shortcite{leclair2020improved}) &
            0.9\%
            \\ 
        \cline{2-6}      
            & 
            H3 - Hu et al.~\shortcite{hu2018summarizing} & 
            BLEU & 
            49.1\% (SPT-Code~\shortcite{spt-code})& 
            48.29\% (AST-Trans~\shortcite{tang2022ast}) &
            1.6\%
            \\ 
        \cline{2-6}    
            & 
            M1 - Miceli et al.~\shortcite{miceli2017parallel} & 
            BLEU & 
            36.1\% (SPT-Code~\shortcite{spt-code})& 
            34.72\% (AST-Trans~\shortcite{tang2022ast}) &
            2.1\%
            \\ 
        \hline  
            \multirow{2}{*}{MN} &
            A2 - Allamanis et al.~\shortcite{allamanis2016convolutional} & 
            F1 & 
            60.15\% (TreeBERT~\shortcite{treebert}) & 
            57.54\% (Code+GNN+GRU~\shortcite{leclair2020improved}) &
            6.1\%
            \\ 
        \cline{2-6}       
            & 
            E1 - ETH Py150~\shortcite{raychev2016probabilistic} & 
            F1 & 
            39.04\% (TreeBERT~\shortcite{treebert}) & 
            34.45\% (Code+GNN+GRU~\shortcite{leclair2020improved}) &
            7.0\%
            \\ 
        \hline 
            CG &
            C5 - CONCODE~\shortcite{iyer2018mapping} & 
            Acc & 
            22.3\% (CodeT5~\shortcite{codet5}) & 
            12.20\% (Iyer et al.~\shortcite{iyer2019learning}) &
            11.5\%
            \\
        \bottomrule
    \end{tabular}
    }
    \caption{Relative error reduction rates on SE tasks. There is no Non-CodePTM approach for CT (Cloze Test).}
    \label{table:sota}
    \vspace{-2mm}
\end{table*}

==> taxonomy_figure.tex <==
\forestset{
    color subtree/.style n args = 2{
        before typesetting nodes = {
            draw = #1,
            fill = #2,
            for descendants = {
                if n children = 0 {draw=none}{draw = #1},
                fill = #2,
            }
        }
    },
    children width/.style = {
        before typesetting nodes = {
            for children = {
                minimum width = #1
            }
        }
    }
}
\begin{figure}[htbp]
    \centering
    \begin{adjustbox}{width=\linewidth}
    \begin{forest}
        for tree = {
            draw = black,
            rounded corners = 2,
            line width = 0.5pt,
            grow' = 0,
            edge = {black, line width = 0.5pt},
            parent anchor = east,
            child anchor = west,
            if = {n_children == 0}{
                draw = none,
                for parent={
                    calign = child edge, 
                    calign child = 1
                }
            }{
                forked edges
            },
        }
        [CodePTMs, fill=gray!10, children width={6em}, calign=child edge, calign child=3,
            [Architecture, color subtree={cyan}{cyan!10}, children width={9.5em}, calign=child edge, calign child=2,
                [LSTM
                    [{SCELMo~\shortcite{scelmo}, CodeDisen~\shortcite{codedisen}}]
                ]
                [Transformer Encoder
                    [{CuBERT~\shortcite{cubert}, CodeBERT~\shortcite{codebert}, C-BERT~\shortcite{c-bert},\\ GraphCodeBERT~\shortcite{graphcodebert}, CugLM~\shortcite{cuglm}, JavaBERT~\shortcite{javabert},\\OSCAR~\shortcite{oscar}, SynCoBERT~\shortcite{syncobert}}, align=left]
                ]
                [Transformer Decoder
                    [GPT-C~\shortcite{gpt-c}]
                ]
                [Transformer
                    [{DOBF~\shortcite{dobf}, T5-learning~\shortcite{t5-learning}, PLBART~\shortcite{plbart},\\ ProphetNet-Code~\shortcite{prophetnet-code}, CoTexT~\shortcite{cotext}, DeepDebug~\shortcite{deepdebug},\\TreeBERT~\shortcite{treebert}, CodeT5~\shortcite{codet5}, SPT-Code~\shortcite{spt-code}}, align=left]
                ]
            ]
            [Modality, color subtree={red}{red!10}, children width={5.5em}, calign=child edge, calign child=2,
                [Unimodal
                    [{CuBERT~\shortcite{cubert}, SCELMo~\shortcite{scelmo}, GPT-C~\shortcite{gpt-c}, C-BERT~\shortcite{c-bert},\\CugLM~\shortcite{cuglm}, JavaBERT~\shortcite{javabert}, DOBF~\shortcite{dobf}, DeepDebug~\shortcite{deepdebug}}, align=left]
                ]
                [Bimodal, children width={9em}, calign=child edge, calign child=1,
                    [Code-NL
                        [{CodeBERT~\shortcite{codebert}, CoTexT~\shortcite{cotext},\\T5-learning~\shortcite{t5-learning}, PLBART~\shortcite{plbart},\\ CodeT5~\shortcite{codet5}, ProphetNet-Code~\shortcite{prophetnet-code}}, align=left]
                    ]
                    [Code-Structure
                        [{TreeBERT~\shortcite{treebert}, OSCAR~\shortcite{oscar}, CodeDisen~\shortcite{codedisen}}]
                    ]
                ]
                [Multimodal, children width={9em}
                    [Code-NL-Structure
                        [{GraphCodeBERT~\shortcite{graphcodebert}, SynCoBERT~\shortcite{syncobert},\\SPT-Code~\shortcite{spt-code}}, align=left]
                    ]
                ]
            ]
            [Task, color subtree={blue}{blue!10}, children width={9em}, calign=child edge, calign child=2,
                [Code-Aware, children width={3.5em}, calign=child edge, calign child=2,
                    [IMLM
                        [{CugLM~\shortcite{cuglm}, DOBF~\shortcite{dobf}, CodeT5~\shortcite{codet5}}, align=left]
                    ]
                    [IT
                        [{CodeT5~\shortcite{codet5}, SynCoBERT~\shortcite{syncobert}}]
                    ]
                    [CCL
                        [{OSCAR~\shortcite{oscar}}]
                    ]
                ]
                [Structure-Aware, children width={3.5em}, calign=child edge, calign child=2,
                    [EP
                        [{GraphCodeBERT~\shortcite{graphcodebert}}]
                    ]
                    [NOP
                        [{TreeBERT~\shortcite{treebert}}]
                    ]
                    [TEP
                        [{SynCoBERT~\shortcite{syncobert}}]
                    ]
                ]
                [Cross-Modal-Aware, children width={9em}, calign=child edge, calign child=2,
                    [Code-NL, children width={4em}
                        [BDG
                            [{CodeT5~\shortcite{codet5}}]
                        ]
                        [MNG
                            [{SPT-Code~\shortcite{spt-code}}]
                        ]
                    ]
                    [Code-Structure, children width={4em}, calign=child edge, calign child=3,
                        [NA
                            [{GraphCodeBERT~\shortcite{graphcodebert}}]
                        ]
                        [TMLM
                            [{TreeBERT~\shortcite{treebert}}]
                        ]
                        [CLR
                            [{CodeDisen~\shortcite{codedisen}}]
                        ]
                        [ACP
                            [{CodeDisen~\shortcite{codedisen}}]
                        ]
                        [CAP
                            [{SPT-Code~\shortcite{spt-code}}]
                        ]
                    ]
                    [Code-NL-Structure, children width={4em}
                        [MCL
                            [{SynCoBERT~\shortcite{syncobert}}]
                        ]
                    ]
                ]
            ]
            [Language, color subtree={teal}{teal!10}, children width={6em}
                [Monolingual, children width={5em},% calign=child edge, calign child=2,
                    [JavaScript
                        [{SCELMo~\shortcite{scelmo}}]
                    ]
                    [C/C++
                        [{C-BERT~\shortcite{c-bert}, OSCAR~\shortcite{oscar}}]
                    ]
                    [Python
                        [{CuBERT~\shortcite{cubert}}]
                    ]
                    [Java
                        [{JavaBERT~\shortcite{javabert}, T5-learning~\shortcite{t5-learning}, DeepDebug~\shortcite{deepdebug}}]
                    ]
                ]
                [Multilingual
                    [{CodeBERT~\shortcite{codebert}, GPT-C~\shortcite{gpt-c}, GraphCodeBERT~\shortcite{graphcodebert}, CugLM~\shortcite{cuglm},\\DOBF~\shortcite{dobf}, PLBART~\shortcite{plbart}, ProphetNet-Code~\shortcite{prophetnet-code}, CoTexT~\shortcite{cotext},\\TreeBERT~\shortcite{treebert}, CodeDisen~\shortcite{codedisen}, CodeT5~\shortcite{codet5}, SynCoBERT~\shortcite{syncobert},\\SPT-Code~\shortcite{spt-code}}, align=left]
                ]
            ]
        ]
    \end{forest}
    \end{adjustbox}
    \caption{Taxonomy for existing CodePTMs.}
    \label{figure:taxonomy}
\end{figure}

==> taxonomy_table.tex <==
\begin{table*}[htbp]
    \centering
    \caption{Taxonomy and list of existing CodePTMs.}
    \label{table:taxonomy}
    \resizebox{\textwidth}{!}{
    \begin{threeparttable}
    \begin{tabular}{l|l|l|l|l|lllll}
        \toprule
            \textbf{Architecture}\tnote{$\ast$} 
            & \multicolumn{2}{l|}{\textbf{Modality}\tnote{$\dagger$}}
            & \textbf{Pre-Training Task}\tnote{$\dagger$}
            & \textbf{Language}\tnote{$\ddagger$}
            & \textbf{CodePTM}
            & \textbf{Input}\tnote{$\S$}
            & \textbf{Objective}\tnote{$\P$}
            & \textbf{Dataset}
            & \textbf{Dataset Size} \\
        \midrule
            \multirow{2}{*}{LSTM}        & \multicolumn{2}{l|}{Unimodal}                          & NLP                        & Mono.                   & SCELMo~\shortcite{scelmo}                   & Code                   & BiLM                                  & JavaScript Open Source Projects                                                         & 150K Files                                                                               \\ \cline{2-10}
                                         & Bimodal                     & C, S                     & C-S                        & Multi.                  & CodeDisen~\shortcite{codedisen}             & Code + AST Seq         & VGVAE + CLR + PD + ACP                & CLCDSA~\shortcite{nafi2019clcdsa}                                                       & 26K Functions                                                                            \\
        \hline
            \multirow{9}{*}{Trans. Enc.} & \multicolumn{2}{l|}{\multirow{4}{*}{Unimodal}}         & \multirow{3}{*}{NLP}       & \multirow{3}{*}{Mono.}  & CuBERT~\shortcite{cubert}                   & Code                   & MLM + NSP                             & Python from BigQuery                                                                    & 7.4M Files                                                                               \\ \cline{6-10}
                                         & \multicolumn{2}{l|}{}                                  &                            &                         & C-BERT~\shortcite{c-bert}                   & Code                   & WWM                                   & C GiHub Repos                                                                           & 5.8GB                                                                                    \\ \cline{6-10}
                                         & \multicolumn{2}{l|}{}                                  &                            &                         & JavaBERT~\shortcite{javabert}               & Code                   & MLM                                   & Java GitHub Repos                                                                       & 3M Files                                                                                 \\ \cline{4-10}
                                         & \multicolumn{2}{l|}{}                                  & NLP, C                     & Multi.                  & CugLM~\shortcite{cuglm}                     & Code                   & IMLM + NSP + Forward LM               & Java, TS GitHub Repos                                                                   & 617K Files                                                                               \\ \cline{2-10}
                                         & \multirow{2}{*}{Bimodal}    & C, N                     & NLP                        & Multi.                  & CodeBERT~\shortcite{codebert}               & Code + Doc             & MLM \& RTD                            & CodeSearchNet                                                                           & \begin{tabular}[c]{@{}l@{}}2.1M Bimodal Functions\\ 6.4M Unimodal Functions\end{tabular} \\ \cline{3-10}
                                         &                             & C, S                     & NLP, C                     & Mono.                   & OSCAR~\shortcite{oscar}                     & IR + AEI               & MLM + CCL                             & C/C++ GitHub Repos                                                                      & 500K functions                                                                           \\ \cline{2-10}
                                         & \multirow{2}{*}{Mulitmodal} & \multirow{2}{*}{C, N, S} & NLP, C-S                   & Multi.                  & GraphCodeBERT~\shortcite{graphcodebert}     & Code + Doc + DFG Nodes & MLM + EP + NA                         & Bimodal CodeSearchNet                                                                   & 2.1M Functions                                                                           \\ \cline{4-10}
                                         &                             &                          & NLP, C, S, C-N-S           & Multi.                  & SynCoBERT~\shortcite{syncobert}             & Code + Doc + AST Seq   & MLM + IT + TEP + MCL                  & CodeSearchNet                                                                           & 6.4M Functions                                                                           \\
        \hline
            Trans. Dec.                  & \multicolumn{2}{l|}{Unimodal}                          & NLP                        & Multi.                  & GPT-C~\shortcite{gpt-c}                     & Code                   & Forward LM                            & Python, C\#, JS/TS GitHub Repos                                                         & 4.7M Files                                                                               \\
        \hline
            \multirow{12}{*}{Transformer} & \multicolumn{2}{l|}{\multirow{2}{*}{Unimodal}}         & C                          & Multi.                  & DOBF~\shortcite{dobf}                       & Code                   & Seq2Seq IMLM                          & Java, Python from BigQuery                                                              & 11.5M Files                                                                              \\ \cline{4-10}
                                         & \multicolumn{2}{l|}{}                                  & NLP                        & Mono.                   & DeepDebug~\shortcite{deepdebug}             & Code                   & Seq2Seq MLM                           & Java GitHub Repos                                                                       & 8M Files                                                                                 \\ \cline{2-10}
                                         & \multirow{9}{*}{Bimodal}    & \multirow{8}{*}{C, N}    & \multirow{6}{*}{NLP}       & Mono.                   & T5-learning~\shortcite{t5-learning}         & Code                   & Seq2Seq MLM                           & Java from CodeSearchNet                                                                 & 1.5M Methods                                                                             \\ \cline{5-10}
                                         &                             &                          &                            & \multirow{5}{*}{Multi.} & PLBART~\shortcite{plbart}                   & Code \& Posts          & DAE (masking / deletion / infilling)  & \begin{tabular}[c]{@{}l@{}}Java, Python GitHub Repos\\ StackOverflow Posts\end{tabular} & \begin{tabular}[c]{@{}l@{}}680M Functions\\ 47M Posts\end{tabular}                       \\ \cline{6-10}
                                         &                             &                          &                            &                         & CoTexT~\shortcite{cotext}                   & Code + Doc             & Seq2Seq MLM                           & \begin{tabular}[c]{@{}l@{}}CodeSearchNet\\ Java, Python from BigQuery\end{tabular}      & \begin{tabular}[c]{@{}l@{}}6.4M Functions\\ Unknown\end{tabular}                         \\ \cline{6-10}
                                         &                             &                          &                            &                         & ProphetNet-Code~\shortcite{prophetnet-code} & Code \& Doc            & FNP                                   & Bimodal CodeSearchNet                                                                   & 2.1M Functions                                                                           \\ \cline{4-10}
                                         &                             &                          & NLP, C, C-N                & Multi.                  & CodeT5~\shortcite{codet5}                   & Code + Doc             & Seq2Seq MLM / IT / Seq2seq IMLM / BDG & \begin{tabular}[c]{@{}l@{}}CodeSearchNet\\ C, C\# from BigQuery\end{tabular}            & 8.35M Functions                                                                          \\ \cline{3-10}
                                         &                             & C, S                     & S, C-S                     & Multi.                  & TreeBERT~\shortcite{treebert}               & Code + AST Paths       & TMLM + NOP                            & Java, Python from BigQuery                                                              & 21.3M Files                                                                              \\ \cline{2-10}
                                         & Multimodal                  & C, N, S                  & NLP, C-S, C-N              & Multi.                  & SPT-Code~\shortcite{spt-code}               & Code + Names + AST Seq & CAP \& MASS \& MNG                    & CodeSearchNet                                                                           & 6.4M Functions                                                                           \\
        \bottomrule
    \end{tabular}
    \begin{tablenotes}
        \footnotesize
        \item[$\ast$] ``Trans. Enc.'' means Transformer Encoder and ``Trans. Dec.'' denotes Transformer Decoder.
        \item[$\dagger$] ``C'', ``N'', ``S'' denote code, natural language and structural information respectively. ``NLP'' indicates the NLP pre-training task.
        \item[$\ddagger$] ``Mono.'' denotes monolingual, ``Multi.'' denotes multilingual.
        \item[$\S$] ``+'' indicates that modalities are concatenated as one input instance, while ``\&'' denotes that the each modality is a standalone input instance.
        \item[$\P$] ``+'' means that the losses of multiple tasks are summed and optimized jointly, ``\&'' indicates that multiple tasks are performed sequentially, while ``/'' means that each pre-training task is performed alternately.
    \end{tablenotes}
    \end{threeparttable}
    }
\end{table*}
